AdaEnlight: Energy-aware Low-light Video Stream Enhancement on Mobile Devices

The ubiquity of camera-embedded devices and the advances in deep learning have stimulated various intelligent mobile video applications. These applications often demand on-device processing of video streams to deliver real-time, high-quality services for privacy and robustness concerns. However, the performance of these applications is constrained by the raw video streams, which tend to be taken with small-aperture cameras of ubiquitous mobile platforms in dim light. Despite extensive low-light video enhancement solutions, they are unfit for deployment to mobile devices due to their complex models and and ignorance of system dynamics like energy budgets. In this paper, we propose AdaEnlight, an energy-aware low-light video stream enhancement system on mobile devices. It achieves real-time video enhancement with competitive visual quality while allowing runtime behavior adaptation to the platform-imposed dynamic energy budgets. We report extensive experiments on diverse datasets, scenarios, and platforms and demonstrate the superiority of AdaEnlight compared with state-of-the-art low-light image and video enhancement solutions.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes


==> body/motivation.tex <==
\section{Motivations}
\label{sec:motivation}



% \begin{itemize}
%     \item the limited size of camera aperture and sensor on mobile device \textit{inherently restrict} the overall amount of light that reaches the camera sensor and thereby decrease the signal-to-noise ratio~\cite{};
%     \item the non-professional mobile users inevitably take videos under \textit{sub-optimal lighting conditions}, \eg back-lit, non-uniform illumination, weak light, and extremely dark environments~\cite{};
%     \item the impertinent image sensor sensitivity (ISO) settings on some visual Apps, for brightening photos on low-light environments, even further amplifies the \textit{noise} ~\cite{}.
% \end{itemize}



\subsection{Intractable QoE Demands on Ubiquitous Video Stream Enhancement}
Both identifying and boosting the user demands on the quality of experience (QoE) of ubiquitous video streams are intractable.
Specifically, the first challenge is building the relationship between QoE measurement and the mobile users' satisfaction.
The QoE metrics we intend to adopt aim to capture the quality of the video enhancement process from both the view of \textit{user experience} and \textit{mobile system performance}.
Depart from the existing efforts on adaptive video streaming, which leverage the coarse-grained resolution or bit rate of each frame as the visual quality metrics.
In this paper, we present to optimize the sequential relevance-aware video stream in the pixel level and introduce the following three QoE demands for enhancing the ubiquitous video stream(s) at the mobile user's end:
\begin{itemize}
    \item \textit{Visual Quality}: maximize the fine-grained visual quality $Q$ of the processed video stream, \eg the signal-to-noise ratio $Q_{n}$ of video display, the recognition accuracy specified by the subsequent video applications;
    \item \textit{Resource efficiency}: minimize the \textit{response latency} $T_{en}$ of video enhancement process on diverse deployment devices with tightly limited resource budgets (\eg computation $C_{bgt}$, memory $M_{bgt}$);
    minimize the energy consumption $E_{en}$ imposed by running video enhancement model on the deployment devices.
    \item  \textit{Agility}: minimize the \textit{response latency} $T_{en}$ of video enhancement process on diverse deployment devices with tightly limited resource budgets (\eg computation $C_{bgt}$, memory $M_{bgt}$);
\end{itemize}
%
% Users prefer to maximize $Q$, minimize $T_{en}$, and minimize $E_{en}$.
%
And the second challenge is, none of existing video QoE enhancement techniques can achieve a great tradeoff between real-time processing efficiency and resource efficiency. \TODO{Prof. Zhou, could you please revise this sentence about existing efforts and check the following preliminary experiment settings.}
%
Furthermore, to achieve the above three video QoE enhancement objectives, we evaluate the feasibility of three classes of existing video QoE improvement techniques, \ie video frame-based enhancement methods xx, video stream-based enhancement methods xx, and video frame-based compressed enhancement methods. 
%
As we will show in $\S$~\ref{sec:experiment}, none of them can achieve all of these three QoE objectives.
% \todo{After Xiaochen's experiment, revise description}. 

Given these challenges, we intend to provide a novel solution, \ie ~ \sysname middleware, to be compatible with resource heterogeneity and optimize all of the above three QoE metrics.


% \subsection{Agnostic Energy Impact of Video Enhancement Process}
% 手机上的能耗问题
% Energy conservation is a vital problem for mobile computing systems, while video-based applications always result in massive energy consumption for video processing~\cite{bib:Mobisys17:Huynh}. 
% %
% To this end, Jason \etal introduced the energy conservation benefits of adaptively adjusting the processing fidelity, which also derives a better runtime optimization between the energy conversation and application QoE ~\cite{bib:WMCSA99:Flinn, bib:SOSP99:Flinn}.
% %
% %没有一个好的能耗反馈仪。尤其是，对于不同的硬件， CPU，GPU，AI加速器，能耗会受到不同的影响。能耗预测器的设计空间很大。
% %
% However, it is non-trivial to profile the energy usage of the DNN-based video process for providing exact runtime feedback on \textit{unknown deployment devices} with \textit{agnostic video stream and sequential DNN topology}. 
% %
% This is because the majority of existing energy profiling methods heavily depend on the processing model's topology (\eg model structure, computation path)~\cite{bib:Mobisys18:Liu} and the deployment platform's hardware resource configurations (\eg on-chip memory capability, computation bandwidth)~\cite{bib:CVPR17:Yang, bib:TCS20:Lee}.
% %
% That is, existing DNN energy usage profiling methods cannot work well for the agnostic runtime optimization of the DNN models over various deployment devices.
% %
% %换言之，我们期望的通过能耗预测来自适应地调整深度模型的计算复杂度，然而一旦深度模型结构在运行时变化了，则基于回归的能耗预测方法也就失效了。
% %
% Once the video process model or deployment device changes at runtime, the pre-defined energy profiling method will fail to provide the precise energy prediction.
% %
% However, this work intends to adaptively adjust the video enhancement model's fidelity (\ie computation) according to the runtime prediction results of energy cost at unknown deployment devices. 
% %
% Therefore, a \textit{runtime DNN-aware} and \textit{one-fit-all} energy prediction method is necessary.
% %

In response to this problem, 
%
%什么行为会带来巨大的能耗降低？降低帧率 or 提升帧复用程度。
%（1）采用不同的输入帧率，采用固定的增强算法 ，播放视频。测试完整pipeline能耗
%（2）帧率不变，采用不同的算法中三种帧复用超参数，播放视频。测试完整pipeline能耗。
% 组合优化（帧率 + 处理模块的复用超参数），得到最优的QoE  & Energy
%
% However, it is non-trivial to profile and predict the energy usage of video QoE enhancement models on various devices at runtime.
%
% 尽管深度模型拓扑在运行时具有动态性，它底层的tensor计算循环是稳定的。
%
%
%
% We defer more details to $\S$ \ref{sec:energy}.

However, it is non-trivial to profile the energy usage of the DNN-based video process for providing exact runtime feedback on \textit{unknown resource availability} with \textit{agnostic video stream and DNN topology}. 
%
The majority of existing energy profiling methods heavily depend on the processing model's topology (\eg model structure, computation path)~\cite{bib:Mobisys18:Liu} and the deployment platform's hardware resource configurations (\eg on-chip memory capability, computation bandwidth)~\cite{bib:CVPR17:Yang, bib:TCS20:Lee}.
%
% They cannot work well for the agnostic runtime optimization of the DNN models over various deployment devices.
%
%换言之，我们期望的通过能耗预测来自适应地调整深度模型的计算复杂度，然而一旦深度模型结构在运行时变化了，则基于回归的能耗预测方法也就失效了。
%
That is, once the video process models or deployment devices change at runtime, the above pre-defined energy profiling methods will fail to provide the precise energy prediction.
%
However, this work intends to adaptively adjust the video enhancement model's computation according to the run-time prediction results of energy cost at unknown deployment devices. 
%
Therefore, a \textit{runtime DNN-aware} and \textit{one-fit-all} energy prediction method is necessary.

Depart from the above methods, \sysnameposs profile the DNN energy based on the following two experimental observations:
\textit{(i)} despite the dynamic topology of video processing models, the underlying tensor operation (\ie the energy-dominating operation loops) and the data flow are stable.
%
% As shown in Figure xx, \todo{to add and describe figure}.
%
\textit{(ii)} In spite of the dynamic hardware resource supply (\eg on-chip memory capability, computation bandwidth), the hit ratio of on-chip memory access shows up the stable rules and within a small sampling set.
